Non-uniform complexity via non-wellfounded proofs

Cyclic and non-wellfounded proofs are now increasingly employed to establish metalogical results in a variety of settings, in particular for type systems with forms of (co)induction. Under the Curry-Howard correspondence, a cyclic proof can be seen as a typing derivation 'with loops', closer to low-level machine models, and so comprise a highly expressive computational model that nonetheless enjoys excellent metalogical properties. In recent work, we showed how the cyclic proof setting can be further employed to model computational complexity, yielding characterisations of the polynomial time and elementary computable functions. These characterisations are 'implicit', inspired by Bellantoni and Cook's famous algebra of safe recursion, but exhibit greater expressivity thanks to the looping capacity of cyclic proofs. In this work we investigate the capacity for non-wellfounded proofs, where finite presentability is relaxed, to model non-uniformity in complexity theory. In particular, we present a characterisation of the class $\mathsf{FP/poly}$ of functions computed by polynomial-size circuits. While relating non-wellfoundedness to non-uniformity is a natural idea, the precise amount of irregularity, informally speaking, required to capture $\mathsf{FP/poly}$ is given by proof-level conditions novel to cyclic proof theory. Along the way, we formalise some (presumably) folklore techniques for characterising non-uniform classes in relativised function algebras with appropriate oracles.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> app-garbage.tex <==
\section{Old stuff, maybe to be deleted}

\subsection{Basic ideas: a warm-up with Cobham}
\todo{I will rework this section to remove the use of Cobham, but rather work with $\fptime$ explicitly.}
As a warm-up, we shall work with a variation of Cobham's algebra based on bounded recursion to motivate the later implicit algebras and systems.

\paragraph*{Sorts}
In order to better control complexity, it will be useful to distinguish a sort $B$ for binary strings (elements of $\{0,1\}^*$) and $N$ for natural numbers (intuitively varying over lengths of words).
We also include a sort $B$ for the Booleans (either $0$ or $1$).
For convenience, we shall assume the natural inclusions $B\subseteq W$ and $N\subseteq W$ by identifying each natural number $n$ with the binary string $\overbrace{1 \cdots 1}^n$.

We shall write $\sigma, \tau,$ etc.\ to vary over sorts.
\paragraph*{Basic functions}
We shall assume an adequate set of initial functions for our purposes.
I presume the following suffice:

\begin{itemize}
	\item A constructor $\succ N{} : N \to N$ by $\succ N{} (n) = n+1$. We shall simply write $\succ{}{} n$ instead of $\succ n{} (n)$.
	\item A constructor $\succ W{} : B \times W \to W$ by $\succ W{} (i, w) = wi$, for $i\in \{0,1\}$.
	We shall simpy write $\succ W i x$ or even $\succ{} i x$ instead of $\succ W{} (i ,x)$, for $i\in \{0,1\}$.\footnote{Note that, formally speaking, this constructor subsumes the previous one on $N$ in the case when $i=1$, by the aforementioned inclusions, but we keep them separate for expositional reasons.}
	\item A destructor $\pred : W \to W$ by:
	$$
	\begin{array}{r@{\ = \ }l}
		\pred (\epsilon) & \epsilon \\
		\pred (\succ{} i x ) & x
	\end{array}
	$$
	\item Projections $\pi_k : \sigma_0 \times \cdots \times \sigma_{n-1} \to \sigma_k$ by $\pi_k(x_0, \dots, x_{n-1}) = x_i$, for $i<n$.
	\item Equality tests $\Eq:\sigma \times \sigma \to B$ for each sort $\sigma$, with:
	$$
	\Eq (x,y) = \begin{cases}
		1 & x=y\\
		0 & x\neq y
	\end{cases}
	$$
	\item Conditionals $\Cnd : B \times \sigma \times \sigma \to \sigma $ for each sort $\sigma$, with:
	$$
	\Cnd (b,x,y) = \begin{cases}
		x & b=0 \\
		y & b=1
	\end{cases}
	$$
	\item A function $\head : W \to B$.
	\item A function $\tail : W \to W$.
	\item A function $\length \cdot : W \to N$, by $\length{b_{n-1}\cdots b_0} = n$.
	\item A function $\times : N \times N \to N$ computing multiplication of two natural numbers. Note that, since we represent natural numbers in unary, this function has same growth rate as $\#$, and so gives us access to arbitrary polynomial bounds.
\end{itemize} 



\paragraph*{Closure operations}
We sometimes indicate the output type of a function in superscript.

The algebra $\Cob$ of functions is the smallest set of functions containing the basic functions of the previous subsection and are closed under:
\begin{itemize}
	\item Composition. If $f^\tau(\vec x,y^\sigma, \vec z) \in \Cob$ and $g^\sigma(\vec x,\vec z) \in \Cob$ then $f(\vec x,g(\vec x,\vec z),\vec z) \in \Cob$.
	\item Bounded recursion on construction. If $g^\sigma(\vec x)\in \Cob$ and $h^\sigma(x,\vec x,y) \in \Cob$ and $k^N(x,\vec x)\in \Cob$ then also $f(x,\vec x) \in \Cob$ where:
	$$
	\begin{array}{r@{\ = \ }ll}
		f(\epsilon,\vec x) & g(\vec x) & \\
		f(x,\vec x) & h(x,\vec x, f(\pred x ,\vec x)) & x\neq \epsilon
	\end{array}
	$$
	as long as $\length{f(x,\vec x) }\leq k(x,\vec x)$.
\end{itemize}

Note that our composition operator is typed, and in particular inputs of sort $B$ or $N$ may be used as inputs of type $W$, under the aforementioned inclusion of sorts $B\subseteq W$ and $N\subseteq W$.
On the other hand, our form of bounded recursion is essentially the adaptation of Cobham's bounded recursion on notation to multiple data structures with different constructors, similar to Leivant's free algebraic approach in his `intrinsic theories'.
In all cases the notion of length is canonical, measuring the number of applications of a constructor.

\paragraph*{Bounding lemma}

Given functions $\vec a$ (of any type), let us write $\Cob(\vec a)$ for the smallest class of functions containing $\Cob$, $\vec a$ and still closed under typed composition and bounded recursion on construction.
We may write functions explicitly indicating such oracles, e.g.\ $f(\vec a)(\vec x)$.
We shall need the following lemma:

\begin{lem}
	Suppose $\vec a = \{a_i\}_{i \in I}$ have polynomial growth rate, i.e.\ there are polynomials $p_i(\vec n)$ with $\length{a_i(\vec x)} \leq p_i(\length {\vec x})$.
	Then, for any $f(\vec a)(\vec x) \in \Cob(\vec a)$ there is a polynomial $p_f(\vec n)$ such that:
	\begin{enumerate}
		\item $\length{f(\vec a)(\vec x)}< p_f(\length{\vec x})$ (polynomial modulus of growth) ; and,
		\item $f(\vec a)(\vec x) = f\left(\lambda \length{\vec x_i} < p_f(\length{\vec x}). a_i(\vec x_i) \right)_{i \in I} (\vec x)$ (polynomial modulus of continuity).
	\end{enumerate}
\end{lem}
\begin{proof}
	[Proof sketch]
	The two properties are proved simultaneously by induction on the definition of $f(\vec a)$.
	The base cases, for initial functions, are immediate with (1) in the case of oracles $a_i$ following by assumption on their growth rate.
	For composition, (1) follows by closure of polynomials under composition, and (2) follows either by assumption (if an oracle is the inner function) or by inductive hypothesis for (1) (if an oracle is the outer function) or both.
	For bounded recursion, we define a suitable polynomial by induction on length.
\end{proof}

Of course, from here, it is routine to establish Cobham's characterisation:

\begin{proposition}
	$\Cob (\vec a) = \fptime (\vec a)$
\end{proposition}

\paragraph*{A characterisation of P/poly}
Let $\vec r = \{r_i\}_{i \in \RR}$ be the class of all relations on natural numbers, so with types of form $r_i : \vec N \to B$.


\begin{proposition}
	$\Cob(\vec r) = \FPpoly$.
\end{proposition}
\begin{proof}
	[Proof sketch]
	Let $f(\vec r)(\vec x) \in \Cob(\vec r)$.
	Clearly $\vec r$ have polynomial (even constant) growth rate, since they are relations, so the bounding lemma applies.
	Moreover, since $f$ has a finite definition, it uses only finitely many $r_i$, so there is a finite set $I\subseteq \RR$ and
	 a polynomial $p_f$ s.t.:
	$$
	\begin{array}{rcl}
		\length{f(\vec r)(\vec x)} &< & p_f (\length{\vec x}) \\
		f(\vec r)(\vec x) & = & f\left( \lambda \length{\vec x_i} < p_f(\length{\vec x}) . r_i(\vec x_i) \right)_{i \in I} (\vec x)
	\end{array}
	$$
	Rephrasing this, $f(\vec x)$ is computed in polynomial-time with access to a polynomial-length bitstring, namely of length $|I|p_f(\length{\vec x})$.
	Thus $f(\vec x) \in \FPpoly$.
	
	Now, let $f(\vec x) \in \FPpoly$, which has polynomial-size circuits $\gamma_{\length{\vec x}}$.
	Define an infinite stream $\gamma$ that prefix-free codes the sequence $(\gamma_{\vec n})_{\vec n}$, and it is clear that $f(\vec x)$ is computed in poylnomial-time by a circuit-evaluator with access to the oracle $\gamma$. 
	Since $\gamma $ may be construed simply as a relation $r_\gamma: N \to B$, we have that $f(\vec x) \in \Cob(r_\gamma)\subseteq \Cob(\vec r)$.
\end{proof}




\subsection{bounding stuff for circular systems}

\subsection{A relativised bounding lemma}


\begin{defn}[Canonical bar]\label{defn:canonical-bar}
Let $\der$ be a $\cbc(\RR)$-coderivation. The \emph{canonical bar} of $\der$, written  $X_\der$, is the set of nodes of $\der$ such that, for any branch $B$:
\begin{itemize}
    \item if $B$ is finite then $X_\der$ contains the leaf of $B$ (including oracles);
    \item if $B$ is infinite then $X_\der$ contains the least node $u\in B$ (called \emph{bud}) such that $\der_u=\der_w$ for some $w \in B$ (called \emph{companion}) strictly below $v$.
\end{itemize}
Given a node $v$ below the bar, we define $X_\der(v)$ as the set of buds of $X_\der$  whose companion is strictly below $v$. If $X_\der(v)=\{u_1, \ldots, u_k\}$ with $\der_{u_i}: \sn, \overset{n_i}{\ldots}, \sn,\n, \overset{m_i}{\ldots}, \n \seqar A$, and $\vec a= a_1, \ldots, a_k$ are oracles with $a_i(x_1, \ldots,x_{n_i}; y_1, \ldots,y_{m_i})$, we denote with  $v(\vec{a})$ the $\cbc(\RR, \vec{a})$-coderivation obtained from $\der_v$ by replacing each $\der_{u_i}$ with the initial sequent $a_i$.
\end{defn}

Notice that the canonical bar of a $\cbc(\RR)$ is a bar by regularity condition. 

In what follows, we shall employ the notation $\sumlen{\vec x} \dfn \sum |\vec x|$. 
Also, we  shall indicate circularities explicitly by extending  $\cbc(\RR)$ with a new inference rule called $\com$: 
$$
\vlinf{\com}{X'}{\Gamma \Rightarrow A}{\Gamma \Rightarrow A}
$$
where $X'$ is a finite (non-empty) set of nodes. In this presentation, we insist that each companion  is always the conclusion of an instance of $\com$, where $X'$ denotes the set of buds having that companion.  This expedient will allow us to formally 
distinguish cases when a node is a companion from those where it is the conclusion of a standard rule of $\cbc$.

To state and prove the Bounding Lemma, we need some preliminary lemmas.

\begin{lem}\label{lem:preliminary1}
Let $\der$ be a $\cbc(\RR)$-coderivation, and let $v$ be the conclusion of the rule $\com$. There exists a node $v'$  above $v$ such that $\der_{v''}$ has no oracles from $\vec a$ and $\denot{v(\vec a)}(0, \overset{n}{\ldots},0; \vec y)=\denot{v''}(0, \overset{n-1}{\ldots},0; \vec z)$ with $\max |\vec z|\leq \max |\vec y|$.
\end{lem}
\begin{proof}
As a consequence of progressiveness, there is a branch $B$ containing the conclusion of a  $\cnd_\sq$-step above $v$. Let $v'$ be its leftmost premise. \red{todo}      
\end{proof}


\begin{lem}\label{lem:preliminary2}
 
\end{lem}



% \begin{lem}[Bounding Lemma]
% \label{lem:boundinglemma}
%  Let $\der(\vec r)(\vec x;\vec y) \in \cbc(\vec r)$, with    $\vec r\in \mathbb R$. There is a polyomial  $m_\der^{\vec c}(\vec x,\vec y)$ such that:
%  $$
%  \def\arraystretch{1.5}
%  \begin{array}{rcl}
%     |\denot \der(\vec a, \vec r)(\vec x;\vec y)| & \leq &  m_\der^{\vec c}(\vec x,\vec y)    \label{eq:elem-const-max-bound} \\
%     \denot \der(\vec a, \vec r)(\vec x; \vec y)    &  = & \denot \der \left(\lambda \vec x_j.\lambda |\vec y_j| \leq m_\der^{\vec c}(\vec x,\vec y) . r_j(\vec x_j;\vec y_j)\right)_j(\vec x;\vec y) 
%  \end{array}
%  $$
% \end{lem}
% \begin{proof}
%  We  will prove a stronger statement. For any $v$ node of $\der(\vec r)$ below the canonical bar $X_\der$ (see~\Cref{defn:canonical-bar}), and for any $\vec a= a_1, \ldots, a_k$ oracles, there is a   function $m_v^{\vec c}(\vec x,\vec y)$ with,
% $$
% m_v^{\vec c}(\vec x,\vec y) = 
% p_v(\sumlen{\vec x}) +\sum\vec c + \max |\vec y|
% $$
% for a monotone polynomial $p_v(n)$  such that whenever there are constants $\vec c=c_1, \dots, c_k$ such that,
% \begin{equation}
%     \label{eq:oracle-const-max-bound}
%     |a_i (\vec x_i;\vec y_i)| \leq c_i + \sum_{j\neq i} c_j + \max|\vec y_i|
% \end{equation}
% for $1\leq i \leq k$,
% we have:\footnote{To be clear, here we write $|\vec y_i| \leq m_v^{\vec c}(\vec x,\vec y)  $ here as an abbreviation for $\{|y_{ij}| \leq m_v^{\vec c}(\vec x,\vec y)\}_j$.}
% \begin{equation}
%     \label{eq:elem-const-max-bound}
%     |\denot {v(\vec a)}(\vec a, \vec r)(\vec x;\vec y)| \leq m_{v}^{\vec c}(\vec x,\vec y)
% \end{equation}
% \begin{equation}
%     \label{eq:input-bounding-eqn}
%     \def\arraystretch{1.5}
%     \begin{array}{rcl} 
%       \denot {v(\vec a)}(\vec a, \vec r)(\vec x; \vec y)     & = & \denot {v(\vec a)} \left(\lambda \vec x_i.\lambda |\vec y_i| \leq m_{v(\vec a)}^{\vec c}(\vec x,\vec y) . a_i(\vec x_i;\vec y_i)\right)_i(\vec x;\vec y) \\
%         \denot {v(\vec a)}(\vec a, \vec r)(\vec x; \vec y)    &  = & \denot {v(\vec a)} \left(\lambda \vec x_j.\lambda |\vec y_j| \leq m_{v(\vec a)}^{\vec c}(\vec x,\vec y) . r_j(\vec x_j;\vec y_j)\right)_j(\vec x;\vec y)
%     \end{array}
% \end{equation}
% where $v(\vec a)$ is as in~\Cref{defn:canonical-bar}.



% We show both with~\Cref{eq:elem-const-max-bound} and~\Cref{eq:input-bounding-eqn} by simultaneous induction on the longest distance of $v$. \todo{Gianluca: notice that in this setting we really need simultaneous induction.}

% If $v$ is a leaf then $p_\der(n)  \dfn 1 +  n$. In particular, if  $v$ is an oracle  $r_i$ then $f_{v(\vec  a)} (\vec x;\vec y) = r_i(\vec x;\vec y)\in \{0,1\}$ and it suffices to set $p_v(n) \dfn 0$.   If $v$ is a bud then $f_{v(\vec  a)} (\vec x;\vec y) = a_i(\vec x;\vec y)$ then it suffices to set $p_v(n) \dfn 0 $.   In all such cases both~\Cref{eq:elem-const-max-bound} and~\Cref{eq:input-bounding-eqn} are immediate.

% The cases where $v$ is the conclusion of $\wk_{\sn}, \wk_\n, \exch,\sql, \sqr , \suc i$ are straightforward. 

% If $\der_v$ has been obtained from $\der_{v'}$, $\der_{v_0}$ and $\der_{v_1}$ by applying the rule $\cnd_{\sn}$ or $\cnd_\n$ then $\denot {v(\vec a)}(0, \vec x; \vec y)= \denot {v'(\vec a)}(\vec x; \vec y)$ and $\denot {v(\vec a)}(\suc i x, \vec x; \vec y)=\denot {v_i(\vec a)}(x, \vec x; \vec y)$. Let $p_{v'}$, $p_{v_0}$, $p_{v_1}$ be obtained from the inductive hypothesis. It suffices to set $p_v(n)\dfn p_{v'}(n)+p_{v_0}(n)+p_{v_1}(n)$.


% If $\der_v$ has been obtained from $\der_{v'}$ and $\der_{v''}$ by applying  the rule  $\cut_\n$, then $\denot {v(\vec a)}(\vec x;\vec y) = \denot {v''(\vec a)}(\vec x;\vec y, \denot {v'(\vec a)}(\vec x;\vec y))$. Let $p_{v'}$  and $p_{v''}$ be obtained from the inductive hypothesis.  We have:
% $$
% \arraycolsep=2pt
% \begin{array}{rcl}
%     |\denot {v(\vec a)}(\vec x;\vec y)| & = & |\denot {v''(\vec a)}(\vec x;\vec y, \denot {v'(\vec a)}(\vec x;\vec y))| \\
%     & \leq & p_{v''}(\sumlen{\vec x}) + \delta_0\sum\vec c + \max(|\vec y|, |\denot {v'(\vec a)}(\vec x;\vec y)|) \\
%     & \leq & p_{v''}(\sumlen{\vec x}) + \delta_0\sum\vec c + p_{v'}(\sumlen{\vec x}) + \delta_1\sum \vec c + \max|\vec y|
%     % \\
%     % & \leq & (e_h(\sumlen{\vec x}) + e_g(\sumlen{\vec x})) + (d_h+d_g)\sum \vec c + \max |\vec y
% \end{array}
% $$
% where $\delta_0, \delta_1 \in \{0,1\}$. Notice that, by left-leaning,  $\delta_0+\delta_1\leq 1$. So we may set $p_v(n) \dfn p_{v'}(n) + p_{v''}(n)$.  Concerning~\Cref{eq:input-bounding-eqn},  by the inductive hypothesis any oracle call only takes safe inputs of lengths:
%     $$
%     \begin{array}{rll}
%      & \leq & p_{v''}(\sumlen{\vec x}) + \delta_0\sum\vec c + \max(|\vec y|, |\denot {v'(\vec a)}(\vec x;\vec y)|) \\
%     & \leq & p_{v''}(\sumlen{\vec x}) + \delta_0\sum\vec c + p_{v'}(\sumlen{\vec x}) + \delta_1\sum \vec c + \max|\vec y|\\
%     &\leq & p_v(\sumlen{\vec x})+ \sum \vec c + \max|\vec y| 
%     \end{array}
%     $$

% If $\der_v$ has been obtained from $\der_{v'}$ and $\der_{v''}$ by applying the rule $\cut_\sq$, then  $\denot {v(\vec a)} (\vec x;\vec y) = \denot{v(\vec a)}(\vec x, \denot {v(\vec a)}(\vec x;);\vec y)$. Let  $p_{v'},p_{v'}$ be  obtained from the inductive hypothesis. Note that, by safety condition on $\der$, we must have that $\denot {v' (\vec a)}$ has no oracles in $\vec a$, and so in fact $|\denot {v' (\vec a)}(\vec x;)| \leq p_{v'}(\sumlen{\vec x})$.
% We thus have,
% $$
% \arraycolsep=2pt
% \begin{array}{rcl}
%     |\denot {v(\vec a)} (\vec x;\vec y)| & = & |\denot {v''(\vec a)}(\vec x, \denot {v'(\vec a)}(\vec x;);\vec y)| \\
%      & \leq & p_{v''}(\sumlen{\vec x}, |\denot {v'(\vec a)}(\vec x;)|) + \sum \vec c + \max|\vec y| \\
%      & \leq & p_{v''}(\sumlen{\vec x}, p_{v'}(\sumlen{\vec x})) + \sum \vec c + \max|\vec y| 
% \end{array}
% $$
% so we may set $p_{v}(n)\dfn p_{v''}(n, p_{v'}(n))$. 
% Concerning~\Cref{eq:input-bounding-eqn},  by the inductive hypothesis, any oracle call will only take safe inputs of lengths:
% $$
% \arraycolsep=2pt
% \begin{array}{rlll}
%      & \leq & p_{v''}(\sumlen{\vec x}, |\denot {v'(\vec a)}(\vec x;)|) + \sum \vec c + \max|\vec y| \\
%      & \leq & p_{v''}(\sumlen{\vec x}, p_{v'}(\sumlen{\vec x})) + \sum \vec c + \max|\vec y| \\
%      & \leq & p_v(\sumlen{\vec x})+ \sum \vec c + \max |\vec y|
% \end{array}
% $$


% Finally, if $\der_v$ has been obtained from $\der_{v'}$ by applying $\com$ then $\denot{v(\vec a)}(\vec x; \vec y)= \denot{v'(\vec a)}(\vec x; \vec y)$, and we set $p_v(n) \dfn n\cdot p_{v'}(n)$. We proceed by a sub-induction on $\sumlen{\vec x}$. For the base case, when $\sumlen{\vec x} = 0 $ (and so, indeed, $\vec x = \vec 0$), we apply~\Cref{lem:preliminary1}, so that there exists $v'$ node above $v$ such that $\der_{v''}$ has no oracles from $\vec a$ and $\denot{v(\vec a)}(0, \overset{n}{\ldots},0; \vec y)=\denot{v''}(0, \overset{n-1}{\ldots},0; \vec z)$ with $\max |\vec z|\leq \max |\vec y|$. So we may appeal to the main inductive hypothesis for $v''$ to obtain:
% $$
% \arraycolsep=2pt
% \begin{array}{rcl}
%     |\denot{v(\vec a)}(\vec 0;\vec y)| & = & |\denot {v'}(\vec 0;\vec y)| \\
%         & \leq & p_{v''}(0) + \sum\vec c + \max |\vec z| \\
%         & \leq & p_{v}(0) + \sum\vec c + \max |\vec y|
% \end{array}
% $$
% as required. Let now $\sumlen{\vec x}>0$. By induction hypothesis on~\Cref{eq:input-bounding-eqn} we have:
% $$
%   \denot {v(\vec a)}(\vec a, \vec r)(\vec x; \vec y)      =  \denot {v(\vec a)} \left( \lambda |\vec y_i| \leq m_{v(\vec a)}^{\vec c}(\vec {x_i},\vec y) . a_i(\vec {x_i};\vec y_i)\right)_{a_i\in X_{v}^{v_j}}(\vec x;\vec y)
% $$
% and by~\Cref{lem:preliminary2} we have that $\sumlen{\vec x_i}<\sumlen{\vec x}$, so that by the sub-inductive hypothesis and monotonicity of $p_v$ we have:
% $$
% |f(\vec {x_i};\vec v)| \leq p_v(\sumlen {\vec x} -1) +  \sum \vec c + \max |\vec v|
% $$
% Now we may again appeal to the main inductive hypothesis for $\denot {v(\vec a)} (\vec a)$ by setting $c= p_{v}(\sumlen{\vec x}  -1)$ to be the corresponding constant for $a = \lambda \vec u. \lambda \vec v. f(\vec u;\vec v)$. 
% We thus obtain:
% $$
% \arraycolsep=2pt
% \begin{array}{rclll}
%      |\denot {v(\vec a)} (\vec x;\vec y)| & = & |\denot{v'(\vec a)}(\lambda \vec v . f(\vec {x_i};\vec v))_{i} (\vec x;\vec y)| \\
%          & \leq & p_{v'} (\sumlen{\vec x}) +  c + \sum\vec c + \max |\vec y| & & \text{main IH} \\
%          & \leq & ( p_{v'} (\sumlen{\vec x}) +  p_v(\sumlen{\vec x} -1) ) +\\
%          & &  + \sum\vec c + \max |\vec y| & & \text{def.~of $c$}\\
%          & \leq & p_v(\sumlen{\vec x}) +  \sum \vec c + \max|\vec y| & & \text{def.~of $p_v(n)$}
% \end{array}
% $$

% We proceed by a sub-induction on $\sumlen{\vec x}$.
%  We immediately inherit from the inductive hypothesis the appropriate bound on safe inputs for oracle calls from $\lambda \vec u\permpref \vec x, \lambda \vec v. f(\vec a)(\vec u;\vec v)$.

% Now, recall from the Bounding \Cref{lem:boundinglemma}, whenever $\vec u \permpref \vec x$ (and so $\sumlen{\vec u} < \sumlen{\vec x}$), we have $|f(\vec u;\vec v)| \leq e_f(\sumlen{\vec x}-1) + d_f\sum \vec c + \max |\vec v|$.
% So by setting $c = e_f(\sumlen{\vec x}-1)$ in the inductive hypothesis for $h(\vec a,a)$, with $a = \lambda \vec u\permpref \vec x, \lambda \vec v. f(\vec a)(\vec u;\vec v)$, any oracle call from $h(\vec a,a)$ will only take safe inputs of lengths:
% $$
% \arraycolsep=2pt
% \begin{array}{rlll}
%     \leq & e_h(\sumlen{\vec x}) + d_h e_f(\sumlen{\vec x}-1) + d_h\sum \vec c + \max |\vec y| \\
%     \leq & e_f(\sumlen{\vec x}) + d_f \sum \vec c + \max |\vec y| & & \text{\eqref{eq:bnd-lem-rec-fn-inv}}
% \end{array}
% $$
% \end{proof}



\begin{lem}\label{lem:cb-oracles-fppoly}
 $ \cbc(\mathbb R)\subseteq \FPpoly$.
\end{lem}
\begin{proof}
	Let $\denot \der(\vec r)(\vec x;) \in  \cbc(\vec r)$.	Clearly $\vec r$ have polynomial (even constant) growth rate, since they are relations, so the bounding lemma applies.
	Moreover, since $\denot \der$ has a finite definition, it uses only finitely many $r_i$, so there is a finite set $I\subseteq \RR$ and
	 a polynomial $p_{\der}$ s.t.:
	$$
	\begin{array}{rcl}
		\length{\denot \der(\vec r)(\vec x;)} &< & p_\der (\length{\vec x}) \\
		\denot \der(\vec r)(\vec x;) & = & \denot \der\left( \lambda \length{\vec x_i} < p_\der(\length{\vec x}) . r_i(\vec x_i;) \right)_{i \in I} (\vec x;)
	\end{array}
	$$
	Rephrasing this, $\denot \der (\vec r)(\vec x;)$ is computed in polynomial-time with access to a polynomial-length bitstring, namely of length $|I|p_\der(\length{\vec x})$.
	Thus $\denot \der(\vec x) \in \FPpoly$.
\end{proof}



% It is useful to consider a syntax that allows us to easily represent the sorts $B,N,W$ etc. For this we shall adapt a fragment of the Kleene Algebra syntax from Kuperberg, Pinault and Pous, along with a modality $\Box$ that can be applied to all types.


% \subsection{Types}
% \emph{Types}, written $\sigma, \tau, $ etc., are generated as follows:
% \[
% \sigma,\tau ::=   \ 1 \ | \ (\sigma + \tau) \ | \ (\sigma \times \tau) \ | \ \sigma^* \ | \ \Box \sigma
% \]

% Some examples:
% \begin{itemize}
% 	\item We may construe $B$ as the type $1+1$.
% 	\item We may construe $N$ as the type $1^*$.
% 	\item We may construe $W$ as the type $(1+1)^*$.
% \end{itemize}

% \newcommand{\seqar}{\Rightarrow}
% \subsection{Rules/constants}
% We consider combinators presented as sequent rules, as usual.
% We include identity, structural rules and cut, and the following logical rules:
% \[
% \vlinf{1l}{}{\Gamma, 1  \seqar \tau}{\Gamma \seqar \tau}
% \qquad
% \vlinf{1r}{}{\seqar 1}{}
% \qquad
% \vlinf{\times l}{}{\Gamma, \rho \times \sigma \seqar \tau}{\Gamma, \rho, \sigma  \seqar \tau}
% \qquad
% \vliinf{\times r}{}{\Gamma \seqar \sigma \times \tau}{\Gamma \seqar \sigma }{\Gamma \seqar \tau}
% \]
% \[
% \vliinf{+l}{}{\Gamma, \rho + \sigma \seqar \tau}{\Gamma, \rho \seqar \tau}{\Gamma, \sigma \seqar \tau }
% \qquad
% \vlinf{+r}{\text{\footnotesize $i =0,1$}}{\Gamma \seqar \tau_0 + \tau_1}{\Gamma \seqar \tau_i}
% \]
% \[
% \vliinf{*l}{}{\Gamma , \sigma^*\seqar \tau}{\Gamma \seqar \tau}{\Gamma ,\sigma, \sigma^* \seqar \tau}
% \qquad
% \vlinf{*r}{}{\Gamma \seqar \tau^*}{}
% \qquad
% \vliinf{*r}{}{\Gamma \seqar \tau^*}{\Gamma \seqar \tau}{\Gamma \seqar \tau^*}
% \]
% We also have $S4$-style modal rules:
% \[
% \vlinf{\Box l}{}{\Gamma, \Box \sigma \seqar \tau}{\Gamma, \sigma \seqar \tau}
% \qquad
% \vlinf{\Box r}{}{\Box \Gamma \seqar \Box \tau}{\Box \Gamma \seqar \tau}
% \]



% \subsection{Adapting progressing, safety and left-leaning criteria}
% \begin{itemize}
% 	\item progress: infinitely often principal thread on some $\Box \sigma^*$ .
% 	\item safety: every branch passes only finitely many cuts on a type with $\Box$ occurring in it.
% 	\item left-leaning: every branch goes right at (any) cut only finitely often.
% \end{itemize}

% \subsection{An interpretation into CB}


% \subsection{Adapting access to all relations}

% Basic idea: insist that there are only finitely many subderivations with $*$ on the RHS or more than one of $+$ or $*$ on the LHS. 
% This should divide the proof into the `circular uniform' part, corresponding to a FP computation with oracles, and oracles that have bounded-size output.



% \red{\begin{lemma}
% Let $\der(\vec a, \vec r)(\vec x;\vec y) \in \cbc(\vec a, \vec r)$, with $\vec a = a_1, \dots, a_k$ and $\vec r\in \mathbb R$. There is a function $m_\der^{\vec c}(\vec x,\vec y)$ with,
% \[
% m_\der^{\vec c}(\vec x,\vec y) = 
% p_\der(\sumlen{\vec x}) +\sum\vec c + \max |\vec y|
% \]
% for a monotone polynomial $p_\der(n)$  such that whenever there are constants $\vec c=c_1, \dots, c_k$ such that,
% \begin{equation}
%     \label{eq:oracle-const-max-bound}
%     |a_i (\vec x_i;\vec y_i)| \leq c_i + \sum_{j\neq i} c_j + \max|\vec y_i|
% \end{equation}
% for $1\leq i \leq k$,
% we have:\footnote{To be clear, here we write $|\vec y_i| \leq m_\der^{\vec c}(\vec x,\vec y)  $ here as an abbreviation for $\{|y_{ij}| \leq m_\der^{\vec c}(\vec x,\vec y)\}_j$.}
% \begin{equation}
%     \label{eq:elem-const-max-bound}
%     |\denot \der(\vec a, \vec r)(\vec x;\vec y)| \leq m_\der^{\vec c}(\vec x,\vec y)
% \end{equation}
% \begin{equation}
%     \label{eq:input-bounding-eqn}
%     \def\arraystretch{1.5}
%     \begin{array}{rcl} 
%       \denot \der(\vec a, \vec r)(\vec x; \vec y)     & = & \denot \der \left(\lambda \vec x_i.\lambda |\vec y_i| \leq m_\der^{\vec c}(\vec x,\vec y) . a_i(\vec x_i;\vec y_i)\right)_i(\vec x;\vec y) \\
%         \denot \der(\vec a, \vec r)(\vec x; \vec y)    &  = & \denot \der \left(\lambda \vec x_j.\lambda |\vec y_j| \leq m_\der^{\vec c}(\vec x,\vec y) . r_j(\vec x_j;\vec y_j)\right)_j(\vec x;\vec y)
%     \end{array}
% \end{equation}
% \end{lemma}
% }
